Using Randomized Nystr\"om Preconditioners to Accelerate Variational Image Reconstruction

Model-based iterative reconstruction plays a key role in solving inverse problems. However, the associated minimization problems are generally large-scale, nonsmooth, and sometimes even nonconvex, which present challenges in designing efficient iterative solvers. Preconditioning methods can significantly accelerate the convergence of iterative methods. In some applications, computing preconditioners on-the-fly is beneficial. Moreover, forward models in image reconstruction are typically represented as operators, and the corresponding explicit matrices are often unavailable, which brings additional challenges in designing preconditioners. Therefore, for practical use, computing and applying preconditioners should be computationally inexpensive. This paper adapts the randomized Nystr\"om approximation to compute effective preconditioners that accelerate image reconstruction without requiring an explicit matrix for the forward model. We leverage modern GPU computational platforms to compute the preconditioner on-the-fly. Moreover, we propose efficient approaches for applying the preconditioners to problems with classical nonsmooth regularizers, i.e., wavelet, total variation, and Hessian Schatten-norm. Our numerical results on image deblurring, super-resolution with impulsive noise, and 2D computed tomography reconstruction illustrate the efficiency and effectiveness of the proposed preconditioner.

==> figslatex/SRGaussianFigs.tex <==
%\begin{figure}[H]%[ht]
%    \centering
%    \subfigure[Bike image.]{\includegraphics[width=0.45\linewidth]{Figures/SRGaussian/PSNRlplqIter.pdf}}
%    \subfigure[Bike image.]{\includegraphics[width=0.47\linewidth]{Figures/SRGaussian/PSNRlplqTime.pdf}}
%    \caption{PSNR values versus number of iteration and wall time of different $p$ values for the image super-resolution task. The downsampling factor is $2$. The added salt-and-pepper noise is $5\%$. ``P-'' denotes the use of a preconditioner.}
%    \label{fig:SRGauss:PSNRIterandTime}
%\end{figure}
%
%\begin{figure}[H]%[ht]
%    \centering
%    \includegraphics[width=0.8\linewidth]{Figures/SRGaussian/IterCGlplqTime.pdf}
%    \caption{Number of iterations when running CG of different $p$ values for the  super-resolution task. The downsampling factor is $2$. The legend is identical to \Cref{fig:SRGauss:PSNRIterandTime}.}
%    \label{fig:SRGauss:CGIter}
%\end{figure}

% \begin{figure*}%[ht]
% 	\centering
	
% \begin{tikzpicture}
%     %%%%%%%%%%%%%% p=1 %%%%%%%%%%%%%%,ylabel = $\ell_1-\ell_1$
%         \begin{axis}[at={(0,0)},anchor = north west,
%     xmin = 0,xmax = 250,ymin = 0,ymax = 70, width=0.95\textwidth,
%         scale only axis,
%         enlargelimits=false,
%         %yshift=1.5cm,
%         %xshift=10cm,
%         %outer sep=6pt,
%         %inner sep=-5pt,
%         %axis on top,
%        axis line style={draw=none},
%        tick style={draw=none},
%         axis equal image,
%         xticklabels={,,},yticklabels={,,},
%         %ylabel style={yshift=-0.2cm,xshift=-0.6cm},
%        ]

% \node[inner sep=0pt, anchor = south west] (p1_1) at (0,0) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Noisy.pdf}};
    
% \node at (8,3) {\color{red} Noisy};
    
%  \node[inner sep=2pt, anchor = west] (p1_2) at (p1_1.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Iml1l1_iter_7.pdf}};

% \node at (57,3) {\color{red} $\ell_1-\ell_1$};
% \node at (87,3) {\color{red} $22.87$dB};
    
%     % \draw[-{latex[length = 0.05mm]}, thick,white] (72 + 67, 57)-- (72 +  61, 54);
%     %\scalebox{1}[-1]
    
%  \node[inner sep=1pt, anchor = west] (p1_3) at (p1_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Iml08l1_iter_7.pdf}};
    
%   \node at (107,3) {\color{red} $\ell_{0.8}-\ell_1$};

%   \node at (135,3) {\color{red} $24.08$dB};
 
%  \node[inner sep=1pt, anchor = west] (p1_4) at (p1_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Iml05l1_iter_7.pdf}};
 
%   \node at (156,3) {\color{red} $\ell_{0.5}-\ell_1$};
%   \node at (184,3) {\color{red} $25.26$dB};
 
%  \node[inner sep=1pt, anchor = west] (p1_5) at (p1_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/GT.pdf}};
% \node at (198.5,3) {\color{red} GT};
  
%  \end{axis}

% \end{tikzpicture} 

% \caption{
% The reconstructed bike image at $7$th iteration with different $p$ values for the super-resolution task. The downsampling factor is $2$. The PSNR value is labeled in the right bottom corner of each image. The first and fifth columns are the noisy measurement and the ground truth, respectively.
% }
% \label{fig:SRGauss:RecoImages}
% \end{figure*}


==> fjjwdphbtzhzystddvtgrqryjkfjwdjs/figslatex/SRGaussianFigs.tex <==
%\begin{figure}[H]%[ht]
%    \centering
%    \subfigure[Bike image.]{\includegraphics[width=0.45\linewidth]{Figures/SRGaussian/PSNRlplqIter.pdf}}
%    \subfigure[Bike image.]{\includegraphics[width=0.47\linewidth]{Figures/SRGaussian/PSNRlplqTime.pdf}}
%    \caption{PSNR values versus number of iteration and wall time of different $p$ values for the image super-resolution task. The downsampling factor is $2$. The added salt-and-pepper noise is $5\%$. ``P-'' denotes the use of a preconditioner.}
%    \label{fig:SRGauss:PSNRIterandTime}
%\end{figure}
%
%\begin{figure}[H]%[ht]
%    \centering
%    \includegraphics[width=0.8\linewidth]{Figures/SRGaussian/IterCGlplqTime.pdf}
%    \caption{Number of iterations when running CG of different $p$ values for the  super-resolution task. The downsampling factor is $2$. The legend is identical to \Cref{fig:SRGauss:PSNRIterandTime}.}
%    \label{fig:SRGauss:CGIter}
%\end{figure}

% \begin{figure*}%[ht]
% 	\centering
	
% \begin{tikzpicture}
%     %%%%%%%%%%%%%% p=1 %%%%%%%%%%%%%%,ylabel = $\ell_1-\ell_1$
%         \begin{axis}[at={(0,0)},anchor = north west,
%     xmin = 0,xmax = 250,ymin = 0,ymax = 70, width=0.95\textwidth,
%         scale only axis,
%         enlargelimits=false,
%         %yshift=1.5cm,
%         %xshift=10cm,
%         %outer sep=6pt,
%         %inner sep=-5pt,
%         %axis on top,
%        axis line style={draw=none},
%        tick style={draw=none},
%         axis equal image,
%         xticklabels={,,},yticklabels={,,},
%         %ylabel style={yshift=-0.2cm,xshift=-0.6cm},
%        ]

% \node[inner sep=0pt, anchor = south west] (p1_1) at (0,0) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Noisy.pdf}};
    
% \node at (8,3) {\color{red} Noisy};
    
%  \node[inner sep=2pt, anchor = west] (p1_2) at (p1_1.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Iml1l1_iter_7.pdf}};

% \node at (57,3) {\color{red} $\ell_1-\ell_1$};
% \node at (87,3) {\color{red} $22.87$dB};
    
%     % \draw[-{latex[length = 0.05mm]}, thick,white] (72 + 67, 57)-- (72 +  61, 54);
%     %\scalebox{1}[-1]
    
%  \node[inner sep=1pt, anchor = west] (p1_3) at (p1_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Iml08l1_iter_7.pdf}};
    
%   \node at (107,3) {\color{red} $\ell_{0.8}-\ell_1$};

%   \node at (135,3) {\color{red} $24.08$dB};
 
%  \node[inner sep=1pt, anchor = west] (p1_4) at (p1_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/Iml05l1_iter_7.pdf}};
 
%   \node at (156,3) {\color{red} $\ell_{0.5}-\ell_1$};
%   \node at (184,3) {\color{red} $25.26$dB};
 
%  \node[inner sep=1pt, anchor = west] (p1_5) at (p1_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussian/GT.pdf}};
% \node at (198.5,3) {\color{red} GT};
  
%  \end{axis}

% \end{tikzpicture} 

% \caption{
% The reconstructed bike image at $7$th iteration with different $p$ values for the super-resolution task. The downsampling factor is $2$. The PSNR value is labeled in the right bottom corner of each image. The first and fifth columns are the noisy measurement and the ground truth, respectively.
% }
% \label{fig:SRGauss:RecoImages}
% \end{figure*}


==> fjjwdphbtzhzystddvtgrqryjkfjwdjs/figslatex/UniformDeblurFigs.tex <==
%\begin{figure}[h]
%    \centering
%    \subfigure[Uniform blur.]{\includegraphics[width=0.46\linewidth]{Figures/UniformDeblur/PSNRlplqIter.pdf}\label{fig:UniformDeblur:PSNRIterandTime:uniformIter}}
%    \subfigure[Uniform blur.]{\includegraphics[width=0.45\linewidth]{Figures/UniformDeblur/PSNRlplqTime.pdf}\label{fig:UniformDeblur:PSNRIterandTime:uniformTime}}
%
%    \subfigure[Gaussian blur.]{\includegraphics[width=0.45\linewidth]{Figures/GaussDeblur/PSNRlplqIter.pdf}\label{fig:UniformDeblur:PSNRIterandTime:GaussIter}}
%    \subfigure[Gaussian blur.]{\includegraphics[width=0.47\linewidth]{Figures/GaussDeblur/PSNRlplqTime.pdf}\label{fig:UniformDeblur:PSNRIterandTime:GaussTime}}
%    \caption{PSNR values versus number of iteration and wall time of different $p$ values for the image deblurring task with uniform and Gaussian blurs. The added salt-and-pepper noise is $5\%$. ``P-'' denotes the use of a preconditioner. First (respectively, second)  row is tested on the starfish (respectively, leaves) image.}
%    \label{fig:UniformDeblur:PSNRIterandTime}
%\end{figure}
%
%\begin{figure}[h]
%    \centering
%   \subfigure[Starfish \& uniform blur.]{\includegraphics[width=0.47\linewidth]{Figures/UniformDeblur/IterCGlplqTime.pdf}}
%    \subfigure[Leaves \& Gaussian blur.]{\includegraphics[width=0.47\linewidth]{Figures/GaussDeblur/IterCGlplqTime.pdf}}
%    \caption{Number of iterations when running CG for different $p$ values in the image deblurring task. The legend is identical to \Cref{fig:UniformDeblur:PSNRIterandTime}.}
%    \label{fig:Deblur:CGIter}
%\end{figure}

%\begin{figure}[H]%[ht]
%    \centering
%    \subfigure[Bike image.]{\includegraphics[width=0.45\linewidth]{Figures/SRGaussian/PSNRlplqIter.pdf}}
%    \subfigure[Bike image.]{\includegraphics[width=0.47\linewidth]{Figures/SRGaussian/PSNRlplqTime.pdf}}
%    \caption{PSNR values versus number of iteration and wall time of different $p$ values for the image super-resolution task. The downsampling factor is $2$. The added salt-and-pepper noise is $5\%$. ``P-'' denotes the use of a preconditioner.}
%    \label{fig:SRGauss:PSNRIterandTime}
%\end{figure}
%
%\begin{figure}[H]%[ht]
%    \centering
%    \includegraphics[width=0.8\linewidth]{Figures/SRGaussian/IterCGlplqTime.pdf}
%    \caption{Number of iterations when running CG of different $p$ values for the  super-resolution task. The downsampling factor is $2$. The legend is identical to \Cref{fig:SRGauss:PSNRIterandTime}.}
%    \label{fig:SRGauss:CGIter}
%\end{figure}


% \begin{figure}%[htb]
%     \centering
%     \subfigure[PSNR versus iteration.]{\includegraphics[width=0.45\linewidth]{Figures/GaussDeblur/PSNRlplqIter.pdf}}
%     \subfigure[PSNR versus wall time.]{\includegraphics[width=0.47\linewidth]{Figures/GaussDeblur/PSNRlplqTime.pdf}}
%     \caption{Comparison of different $p$ values for the leaves image with Gaussian blur. The added salt-and-pepper noise is $5\%$. ``P-'' denotes the use of a preconditioner.}
%     \label{fig:GaussDeblur:PSNRIterandTime}
% \end{figure}

% \begin{figure}%[htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figures/GaussDeblur/IterCGlplqTime.pdf}
%     \caption{Number of iterations when running CG of different $p$ values for the leaves image with uniform blur. The legend is identical to \Cref{fig:GaussDeblur:PSNRIterandTime}.}
%     \label{fig:GaussDeblur:CGIter}
% \end{figure}


\begin{figure*}[ht]%[htb]
\vspace{-2cm}
	\centering
\begin{tikzpicture}
    %%%%%%%%%%%%%% p=1 %%%%%%%%%%%%%%,ylabel = $\ell_1-\ell_1$
    \begin{axis}[at={(0,0)},anchor = north west,
    xmin = 0,xmax = 250,ymin = 0,ymax = 70, width=0.95\textwidth,
        scale only axis,
        enlargelimits=false,
        %yshift=1.5cm,
        %xshift=10cm,
        %outer sep=6pt,
        %inner sep=-5pt,
        %axis on top,
       axis line style={draw=none},
       tick style={draw=none},
        axis equal image,
        xticklabels={,,},yticklabels={,,},
        %ylabel style={yshift=-0.2cm,xshift=-0.6cm},
       ]

    \node[inner sep=0pt, anchor = south west] (p1_1) at (0,0) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Noisy.pdf}};
    
    \node at (8,3) {\color{white} Noisy};
    
     \node at (22,44) {\color{white} Deblurring, Uniform};
     
    \node[inner sep=2pt, anchor = west] (p1_2) at (p1_1.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml1l1_iter_10.pdf}};

    \node at (57,3) {\color{white} $\ell_1-\ell_1$};
    \node at (88,3) {\color{white} $30.7$dB};
    % \node at (87,3) {\color{white} $30.75$dB};
    
    % \draw[-{latex[length = 0.05mm]}, thick,white] (72 + 67, 57)-- (72 +  61, 54);
    %\scalebox{1}[-1]
    
    \node[inner sep=1pt, anchor = west] (p1_3) at (p1_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml08l1_iter_10.pdf}};
    
   \node at (107,3) {\color{white} $\ell_{0.8}-\ell_1$};
    \node at (137,3) {\color{white} $34.2$dB};
  % \node at (135,3) {\color{white} $34.18$dB};
 \node[inner sep=1pt, anchor = west] (p1_4) at (p1_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml05l1_iter_10.pdf}};
 
  \node at (156,3) {\color{white} $\ell_{0.5}-\ell_1$};
  \node at (186,3) {\color{white} $38.4$dB};
  % \node at (184,3) {\color{white} $38.39$dB};
 \node[inner sep=1pt, anchor = west] (p1_5) at (p1_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/GT.pdf}};
\node at (198.5,3) {\color{white} GT};
  
 \end{axis}

\begin{axis}[at={(p1_1.south west)},anchor = north west,
    xmin = 0,xmax = 250,ymin = 0,ymax = 70, width=0.95\textwidth,
        scale only axis,
        enlargelimits=false,
        yshift=1.5cm,
        %xshift=10cm,
        %outer sep=6pt,
        %inner sep=-5pt,
        %axis on top,
       axis line style={draw=none},
       tick style={draw=none},
        axis equal image,
        xticklabels={,,},yticklabels={,,},
        %ylabel style={yshift=-0.2cm,xshift=-0.6cm},
       ]

\node[inner sep=0pt, anchor = south west] (Gaussp1_1) at (0,0) {\includegraphics[ width=0.18\textwidth]{Figures/GaussDeblur/Noisy.pdf}};
    
   % \node at (8,3) {\color{red} Noisy};
    \node at (22,44) {\color{black} Deblurring, Gaussian};
 \node[inner sep=2pt, anchor = west] (Gaussp1_2) at (Gaussp1_1.east) {\includegraphics[ width=0.18\textwidth]{Figures/GaussDeblurNew/Iml1l1_iter_6.pdf}};

\node at (57,3) {\color{black} $\ell_1-\ell_1$};
\node at (88,3) {\color{black} $29.6$dB};
%\node at (87,3) {\color{black} $29.64$dB};    
    % \draw[-{latex[length = 0.05mm]}, thick,white] (72 + 67, 57)-- (72 +  61, 54);
    %\scalebox{1}[-1]
    
 \node[inner sep=1pt, anchor = west] (Gaussp1_3) at (Gaussp1_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/GaussDeblurNew/Iml08l1_iter_6.pdf}};
    
  \node at (107,3) {\color{black} $\ell_{0.8}-\ell_1$};

  \node at (137,3) {\color{black} $31.5$dB};
 %\node at (135,3) {\color{black} $31.48$dB};
 
 \node[inner sep=1pt, anchor = west] (Gaussp1_4) at (Gaussp1_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/GaussDeblurNew/Iml05l1_iter_6.pdf}};
 
  \node at (156,3) {\color{black} $\ell_{0.5}-\ell_1$};
  \node at (186,3) {\color{black} $33.3$dB};

 %\node at (184,3) {\color{black} $33.28$dB};
 \node[inner sep=1pt, anchor = west] (Gaussp1_5) at (Gaussp1_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/GaussDeblurNew/GT.pdf}};
%\node at (198.5,3) {\color{red} GT};
\end{axis}

\begin{axis}[at={(Gaussp1_1.south west)},anchor = north west,
    xmin = 0,xmax = 250,ymin = 0,ymax = 70, width=0.95\textwidth,
        scale only axis,
        enlargelimits=false,
        yshift=1.5cm,
        %xshift=10cm,
        %outer sep=6pt,
        %inner sep=-5pt,
        %axis on top,
       axis line style={draw=none},
       tick style={draw=none},
        axis equal image,
        xticklabels={,,},yticklabels={,,},
        %ylabel style={yshift=-0.2cm,xshift=-0.6cm},
       ]

\node[inner sep=0pt, anchor = south west] (p1_1) at (0,0) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussNew/Noisy.pdf}};
    
%\node at (8,3) {\color{red} Noisy};
   \node at (18,44) {\color{white} Super-Resolution};
 \node[inner sep=2pt, anchor = west] (p1_2) at (p1_1.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussNew/Iml1l1_iter_7.pdf}};

\node at (57,3) {\color{white} $\ell_1-\ell_1$};
\node at (88,3) {\color{white} $22.9$dB};
    %\node at (87,3) {\color{white} $22.87$dB};
    % \draw[-{latex[length = 0.05mm]}, thick,white] (72 + 67, 57)-- (72 +  61, 54);
    %\scalebox{1}[-1]
    
 \node[inner sep=1pt, anchor = west] (p1_3) at (p1_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussNew/Iml08l1_iter_7.pdf}};
    
 \node at (107,3) {\color{white} $\ell_{0.8}-\ell_1$};

  \node at (137,3) {\color{white} $24.1$dB};

 % \node at (135,3) {\color{white} $24.08$dB};
 
 \node[inner sep=1pt, anchor = west] (p1_4) at (p1_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussNew/Iml05l1_iter_7.pdf}};
 
  \node at (156,3) {\color{white} $\ell_{0.5}-\ell_1$};
  \node at (186,3) {\color{white} $25.3$dB};

  %\node at (184,3) {\color{white} $25.26$dB};
 \node[inner sep=1pt, anchor = west] (p1_5) at (p1_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/SRGaussNew/GT.pdf}};
%\node at (198.5,3) {\color{red} GT};
  
 \end{axis}
 
%,ylabel = $\ell_{0.8}-\ell_1$
% \begin{axis}[at={(p1_1.south west)},anchor = north west,
%     xmin = 0,xmax = 100,ymin = 0,ymax = 70, width=0.95\textwidth,
%         scale only axis,
%         enlargelimits=false,
%         yshift=7.8cm,
%         %outer sep=6pt,
%         %inner sep=-5pt,
%         %axis on top,
%        axis line style={draw=none},
%        tick style={draw=none},
%         axis equal image,
%         xticklabels={,,},yticklabels={,,},
%         ylabel style={yshift=-0.2cm,xshift=-0.6cm},
%        ]

%     \node[inner sep=0pt, anchor = south west] (p08_1) at (0,0) {\includegraphics[ width=0.23\textwidth]{Figures/UniformDeblur/Noisy.pdf}};
    
%     \node[inner sep=3pt, anchor = west] (p08_2) at (p08_1.east) {\includegraphics[ width=0.23\textwidth]{Figures/UniformDeblur/Iml08l1_iter_3.pdf}};
    
%     %\node at (52,48) {\color{white} $50$};
%     %\node at (57,3) {\color{red} $30.23$dB};
    
%  %    \node[inner sep=0pt, anchor = west] (p08_3) at (p08_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml08l1_iter_5.pdf}};
 
%  % \node[inner sep=0pt, anchor = west] (p08_4) at (p08_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml08l1_iter_10.pdf}};


%  % \node[inner sep=0pt, anchor = west] (p08_5) at (p08_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/GT.pdf}};
 
%  \end{axis}

%  \begin{axis}[at={(p08_1.south west)},anchor = north west,ylabel = $\ell_{0.5}-\ell_1$,
%     xmin = 0,xmax = 250,ymin = 0,ymax = 70, width=0.95\textwidth,
%         scale only axis,
%         enlargelimits=false,
%         yshift=1.3cm,
%         %outer sep=6pt,
%         %inner sep=-5pt,
%         %axis on top,
%        axis line style={draw=none},
%        tick style={draw=none},
%         axis equal image,
%         xticklabels={,,},yticklabels={,,},
%         ylabel style={yshift=-0.2cm,xshift=-0.6cm},
%        ]

%     \node[inner sep=0pt, anchor = south west] (p05_1) at (0,0) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Noisy.pdf}};
    
%     \node[inner sep=0pt, anchor = west] (p05_2) at (p05_1.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml05l1_iter_3.pdf}};%XY_2

%     \node[inner sep=0pt, anchor = west] (p05_3) at (p05_2.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml05l1_iter_5.pdf}};
    
%  \node[inner sep=0pt, anchor = west] (p05_4) at (p05_3.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/Iml05l1_iter_10.pdf}};

%   \node[inner sep=0pt, anchor = west] (p05_5) at (p05_4.east) {\includegraphics[ width=0.18\textwidth]{Figures/UniformDeblur/GT.pdf}};
%  \end{axis}
 
\end{tikzpicture} 

\caption{
The reconstructed images for different $p$ on the image deblurring (\MRcb{first and second rows}) and super-resolution (\MRcb{third row}) tasks. The PSNR value is labeled at the right bottom corner of each image. The first and fifth columns are the noisy measurement and the ground truth, respectively. The first (respectively, second) row is the reconstructed starfish (respectively, leaves) image at $10$th (respectively, $6$th)  iteration for the image deblurring task with uniform (respectively, Gaussian) blur. The third row is the reconstructed bike image at $7$th iteration for the image super-resolution task with a downsampling factor $2$
and $5$\% salt-and-pepper noise.
}
\label{fig:UniformGaussianDeblurSR:RecoImages}
\end{figure*}


\begin{table*}[t]
    \centering
     \caption{Comparison of PSNR and ST for different $p$ in the image deblurring task with uniform and Gaussian blurs. We ran  \IRM  $20$ iterations on each image and presented the highest PSNR values within these $20$ iterations along with the associated ST values. The highest PSNR and ST values for each image are marked in bold.}
 \setlength\tabcolsep{3.35pt}
\begin{tabular}{p{1cm}||rr|rr|rr|rr|rr|rr|rr|rr|rr}
 %\hline
 %\multicolumn{4}{|c|}{Country List} \\
 
 \hline
 \hline
%\multirow{2}{ 3&4&5&6}\\\diagbox[innerwidth=1.83cm]{$p$}{Image} \multirow{2}*{Image}
Image&\multicolumn{2}{c|}{Butterfly}  & \multicolumn{2}{c|}{Boats}&\multicolumn{2}{c|}{C. Man} &\multicolumn{2}{c|}{House} &\multicolumn{2}{c|}{Parrot}  & \multicolumn{2}{c|}{Barbara} & \multicolumn{2}{c|}{Starfish} & \multicolumn{2}{c|}{Peppers}& \multicolumn{2}{c}{Leaves} \\

\hline

\multicolumn{19}{c}{Deblurring: Uniform blur, 5\% salt-and-pepper noise}
\\
\hline
%\cline{2-19}

& PSNR & ST  & PSNR & ST  &PSNR & ST &PSNR & ST  &PSNR & ST  &PSNR & ST  &PSNR & ST  & PSNR& ST 
&PSNR & ST 

 \\
 \cline{2-19}
 $p=1$  &  $31.6$&$0.94$&
        $32.9$  & $0.94$&
        $31.8$&$0.95$  &
        $35.9$ & $0.93$&
        
        $32.3$&$0.95$&
        $27.9$&$0.95$ &
        
        $30.8$&$0.94$&
        $32.2$ &$0.94$&
         $30.7$ &$0.94$

        %   $31.57$&$0.94$&%12   
        % $32.87$  & $0.94$&%16
        % $31.81$&$0.95$  &%57
        % $35.89$ & $0.93$&%29
        
        % $32.29$&$0.95$&%76
        % $28.00$&$0.95$ &% 22
        
        % $30.82$&$0.94$&%65
        % $32.22$ &$0.94$&%52
        %  $30.65$ &$0.94$%72
 \\

 \hline

 $p=0.8$  &  $35.3$&$0.96$&  
        $35.9$  & $0.95$&
        $35.1$&$0.97$  &
        $38.7$ &  $0.96$&
             
        $35.7$&$0.97$&
        $31.1$&$0.97$ &
        
        $34.2$&$0.96$&
        $35.2$ &$0.96$&
         $34.7$ &$0.96$

        %   $35.35$&$0.96$&   %35
        % $36.03$  & $0.95$&%89
        % $35.11$&$0.97$  &%07
        % $38.74$ &  $0.96$&%06
             
        % $35.69$&$0.97$&%43
        % $31.06$&$0.97$ &% 35
        
        % $34.20$&$0.96$&%98
        % $35.16$ &$0.96$&%34
        %  $34.71$ &$0.96$%43
 \\       
 \hline

 $p=0.5$  &  $\bm{39.9}$&$\bm{0.98}$& 
        $\bm{39.9}$  & $\bm{0.97}$&
        $\bm{38.8}$&$\bm{0.98}$  &  
         $\bm{42.5}$ &  $\bm{0.98}$&

        $\bm{39.2}$&$\bm{0.98}$&
        $\bm{34.9}$&$\bm{0.98}$ &
        
        $\bm{38.4}$&$\bm{0.98}$&
        $\bm{38.8}$ &$\bm{0.98}$&
         $\bm{39.7}$ &$\bm{0.98}$

        %  $\bm{39.96}$&$\bm{0.98}$& 
        % $\bm{39.85}$  & $\bm{0.97}$&
        % $\bm{38.83}$&$\bm{0.98}$  &  
        %  $\bm{42.54}$ &  $\bm{0.98}$&

        % $\bm{39.24}$&$\bm{0.98}$&
        % $\bm{34.89}$&$\bm{0.98}$ &
        
        % $\bm{38.42}$&$\bm{0.98}$&
        % $\bm{38.76}$ &$\bm{0.98}$&
        %  $\bm{39.66}$ &$\bm{0.98}$
 \\
 \hline

 \multicolumn{19}{c}{Deblurring: Gaussian blur, 5\% salt-and-pepper noise}

 \\
 \hline
 
 $p=1$  &  $29.5$&$0.95$&   
        $30.9$  & $0.96$&
        $29.4$&$0.97$  &
        $34.1$ & $0.96$&
        $31.9$&$0.96$&
        $28.1$&$0.97$ &
        $29.9$&$0.96$&
        $31.3$ &$0.95$&
         $29.7$ &$0.96$


        %  $29.54$&$0.95$&   
        % $31.04$  & $0.96$&
        % $29.40$&$0.97$  &
        % $34.12$ & $0.96$&
        % $31.88$&$0.96$&
        % $28.14$&$0.97$ &
        % $29.87$&$0.96$&
        % $31.26$ &$0.95$&
        %  $29.69$ &$0.96$
 \\

 \hline

 $p=0.8$  &  $31.5$  & $0.98$&  
        $32.9$  & $0.98$&
        $31.5$ & $0.98$&
        $35.6$&$0.98$  &
        $33.5$&$0.98$&
        $30.3$&$0.98$ &
        $31.9$&$0.98$&
        $32.5$ &$0.98$&
         $31.5$ &$0.98$

        %  $31.45$  & $0.98$&  
        % $32.93$  & $0.98$&
        % $31.52$ & $0.98$&
        % $35.58$&$0.98$  &
        % $33.53$&$0.98$&
        % $30.25$&$0.98$ &
        % $31.85$&$0.98$&
        % $32.46$ &$0.98$&
        %  $31.50$ &$0.98$
 \\      
 \hline

 $p=0.5$  &  $\bm{33.5}$&$\bm{0.99}$& 
        $\bm{35.2}$  & $\bm{0.99}$&
        $\bm{33.5}$&$\bm{0.99}$  &  
         $\bm{37.4}$ &  $\bm{0.99}$&
        $\bm{34.9}$&$\bm{0.99}$&
        $\bm{31.9}$&$\bm{0.99}$ &
        $\bm{33.7}$&$\bm{0.99}$&
        $\bm{34.1}$ &$\bm{0.99}$&
         $\bm{33.3}$ &$\bm{0.99}$

        %  $\bm{33.47}$&$\bm{0.99}$& 
        % $\bm{35.16}$  & $\bm{0.99}$&
        % $\bm{33.49}$&$\bm{0.99}$  &  
        %  $\bm{37.40}$ &  $\bm{0.99}$&
        % $\bm{34.96}$&$\bm{0.99}$&
        % $\bm{32.04}$&$\bm{0.99}$ &
        % $\bm{33.72}$&$\bm{0.99}$&
        % $\bm{33.95}$ &$\bm{0.99}$&
        %  $\bm{33.28}$ &$\bm{0.99}$

\end{tabular}
    \label{tab:DeblurTable}
\end{table*}


\begin{table*}[t]
    \centering
     \caption{Comparison of PSNR and ST for different $p$ in the image super-resolution task. We ran \IRM $20$ iterations on each image and presented the highest PSNR values within these $20$ iterations along with the associated ST values. The highest PSNR and ST values for each image are marked in bold.}
     \setlength\tabcolsep{3.35pt}
\begin{tabular}{p{1cm}||rr|rr|rr|rr|rr|rr|rr|rr|rr}
 %\hline
 %\multicolumn{4}{|c|}{Country List} \\
 
 \hline
  \hline
 \multicolumn{19}{c}{Super-resolution: scaling = 2, 5\% salt-and-pepper noise}
 \\
 \hline
%\multirow{2}{ 3&4&5&6}\\\diagbox[innerwidth=1.83cm]{$p$}{Image} \multirow{2}*{Image}
\multirow{2}*{Image}&\multicolumn{2}{c|}{Butterfly}  & \multicolumn{2}{c|}{Flower}&\multicolumn{2}{c|}{Girl} &\multicolumn{2}{c|}{Parth.} &\multicolumn{2}{c|}{Parrot}  & \multicolumn{2}{c|}{Racoon} & \multicolumn{2}{c|}{Bike} & \multicolumn{2}{c|}{Hat}& \multicolumn{2}{c}{Plants} \\

\cline{2-19}
% \multicolumn{19}{c}{Deblurring: Uniform blur, 5\% salt-and-pepper noise}
% \\
% \hline
%\cline{2-19}

& PSNR & ST  & PSNR & ST  &PSNR & ST &PSNR & ST  &PSNR & ST  &PSNR & ST  &PSNR & ST  & PSNR& ST 
&PSNR & ST 

 \\
 \hline
 $p=1$  &  $25.6$&$0.74$&   
        $27.4$  & $0.74$&
        $31.6$&$0.78$  &
        $24.5$ & $0.43$&
        $27.5$&$0.76$&
        $27.3$&$0.68$ &
        $23.2$&$0.76$&
        $29.4$ &$0.76$&
        $31.9$ &$0.76$


        %  $25.59$&$0.74$&   
        % $27.36$  & $0.74$&
        % $31.57$&$0.78$  &
        % $24.45$ & $0.43$&
        % $27.54$&$0.76$&
        % $27.31$&$0.68$ &
        % $23.17$&$0.76$&
        % $29.37$ &$0.76$&
        % $31.88$ &$0.76$
 \\

 \hline

 $p=0.8$  &  $27.1$&$0.94$&
        $28.7$  & $0.93$&
        $32.5$&$0.91$  &
        $25.4$ &  $0.91$&
        $28.6$&$0.94$&
        $28.4$&$0.90$ &
        $24.3$&$0.93$&
        $30.3$ &$0.94$&
         $33.3$ &$0.92$

        %  $27.05$&$0.94$&
        % $28.65$  & $0.93$&
        % $32.48$&$0.91$  &
        % $25.43$ &  $0.91$&
        % $28.65$&$0.94$&
        % $28.42$&$0.90$ &
        % $24.34$&$0.93$&
        % $30.31$ &$0.94$&
        %  $33.26$ &$0.92$
 \\       
 \hline

 $p=0.5$  &  $\bm{28.1}$&$\bm{0.96}$&
        $\bm{29.6}$  & $\bm{0.97}$&
        $\bm{33.1}$&$\bm{0.96}$  &  
         $\bm{25.9}$ &  $\bm{0.96}$& 
        $\bm{29.7}$&$\bm{0.97}$&
        $\bm{29.4}$&$\bm{0.97}$ &
        $\bm{25.3}$&$\bm{0.97}$&
        $\bm{31.4}$ &$\bm{0.96}$&
         $\bm{34.4}$ &$\bm{0.96}$

        %   $\bm{28.13}$&$\bm{0.96}$&
        % $\bm{29.55}$  & $\bm{0.97}$&
        % $\bm{33.07}$&$\bm{0.96}$  &  
        %  $\bm{25.88}$ &  $\bm{0.96}$& 
        % $\bm{29.73}$&$\bm{0.97}$&
        % $\bm{29.36}$&$\bm{0.97}$ &
        % $\bm{25.27}$&$\bm{0.97}$&
        % $\bm{31.38}$ &$\bm{0.96}$&
        
        %  $\bm{34.42}$ &$\bm{0.96}$
         \end{tabular}
    \label{tab:SRTable}
\end{table*}


